Unified Video Action Model

A unified video and action model holds significant promise for robotics, where videos provide rich scene information for action prediction, and actions provide dynamics information for video prediction. However, effectively combining video generation and action prediction remains challenging, and current video generation-based methods struggle to match the performance of direct policy learning in action accuracy and inference speed. To bridge this gap, we introduce the Unified Video Action model (UVA), which jointly optimizes video and action predictions to achieve both high accuracy and efficient action inference. The key lies in learning a joint video-action latent representation and decoupling video-action decoding. The joint latent representation bridges the visual and action domains, effectively modeling the relationship between video and action sequences. Meanwhile, the decoupled decoding, powered by two lightweight diffusion heads, enables high-speed action inference by bypassing video generation during inference. Such a unified framework further enables versatile functionality through masked input training. By selectively masking actions or videos, a single model can tackle diverse tasks beyond policy learning, such as forward and inverse dynamics modeling and video generation. Via an extensive set of experiments, we demonstrate that UVA can serve as a general-purpose solution for a wide range of robotics tasks, such as policy learning, forward/inverse dynamics and video observation prediction, without compromising performance compared to methods tailored for specific applications. Results are best viewed on https://unified-video-action-model.github.io/.

==> after_ddl_notes.tex <==


A slide deck for presenting this work: (Shuang think about how you going to present it in your talk)
- include method description. 
- highlight the conclusion + advantages 
- include other task evaluation: as video generator, as planner




Additional experiments: 
- Train our model on all the available umi data for video-action generation.  
- Pretrain video generation on all tasks except these three tasks, then only use 200 episode each for the current three tasks)
- Baseline on push-T: https://dino-wm.github.io/


Before release 
- A colab example for Push-T

==> tables/history_len.tex <==
\begin{table}[t]
\small
  \caption{\small 
         \textbf{Different history length (PushT-Multi).} \shuang{make this a plot}
         }
        \label{tab:historylen}
  % \vspace{-7pt}
  \centering
  % \setlength{\tabcolsep}{0.5em}
  % \scalebox{1}{
  \begin{tabular}{lccccccccc}
    \toprule
    & \bf 1 & \bf 2 & \bf 4 & \bf 8 & \bf 16 \\
    \midrule
    \bf DP-C & 0.68 & 0.63 & 0.59 & 0.40 & 0.19 \\
    \bf Ours & \\
    \bottomrule
  \end{tabular}
  % }
  % \vspace{-10pt}
\end{table}



==> text/background.tex <==
\section{Sequence Modeling Tasks in Robotics}
\label{sec:background}

Given a sequence of states \(\{\mathbf{s}_{t-h}, \cdots, \mathbf{s}_{t}, \cdots, \mathbf{s}_{t+h}\}\) and a sequence of actions \(\{\mathbf{a}_{t-h}, \cdots, \mathbf{a}_{t}, \cdots, \mathbf{a}_{t+h}\}\), our objective is to perform several essential tasks in policy learning, dynamics modeling, and video planning.


\textbf{Policy Learning}.
Policy learning involves determining the optimal mapping from states to actions. Given the history and current state \(\{\mathbf{s}_{t-h}, \cdots, \mathbf{s}_t\}\), the objective is to learn a policy that maximizes cumulative rewards over a sequence. The learned policy can be expressed as:
% \(\pi: \mathbf{s} \to \mathbf{a}\) 
\[
\mathbf{a}_t, \cdots, \mathbf{a}_{t+h} = f_{\text{policy}}(\mathbf{s}_{t-h}, \cdots, \mathbf{s}_{t}).
\]
% where \(\pi\) is the policy model, which can be parameterized using neural networks.

\textbf{Forward Dynamics.}
Forward dynamics modeling predicts the future state of the system given the current state and an action. Formally, it learns a function:
% \(f: (\mathbf{s}_t, \mathbf{a}_t) \to \mathbf{s}_{t+1}\), where:
\[
\mathbf{s}_{t+1} = f_{\text{forward}}(\mathbf{s}_t, \mathbf{a}_t).
\]
This model is essential for tasks such as simulation and planning, where understanding how actions influence state transitions is critical.

\textbf{Inverse Dynamics}.
Inverse dynamics modeling predicts the action that caused the transition from one state to another. It learns a function:
% \(f: (\mathbf{s}_t, \mathbf{s}_{t+1}) \to \mathbf{a}_t\), where:
\[
\mathbf{a}_t = f_{\text{inverse}}(\mathbf{s}_t, \mathbf{s}_{t+1}).
\]
This is crucial for imitation learning and control systems where actions need to be inferred from observed state transitions.

\textbf{Video Planning}.
Given a set of history and current state \(\{\mathbf{s}_{t-h}, \cdots, \mathbf{s}_t\}\), video planning generates a sequence of future states such that:
\[\mathbf{s}_{t+1}, \cdots, \mathbf{s}_{t+h} = f_{\text{video}}(\mathbf{s}_{t-h}, \cdots, \mathbf{s}_{t}).
\]
This task is crucial for predicting and planning the system's future behavior, enabling informed decision-making in scenarios that require anticipating outcomes.



\textbf{Full Dynamics Modeling}.
Full dynamics modeling unifies policy learning and video planning into a comprehensive framework. 
\[\mathbf{a}_t, \mathbf{s}_{t+1}, \cdots, \mathbf{a}_{t+h-1}, \mathbf{s}_{t+h} = f_{\text{full}}(\mathbf{s}_{t-h}, \cdots, \mathbf{s}_{t}).
\]
This comprehensive prediction facilitates holistic planning and control, enabling the system to account for both immediate and long-term outcomes in dynamic environments.



==> text/method_old.tex <==

\input{figs/model.tex}

\section{Unified Video Action Model}
\label{sec:method}

% Previous policy learning methods, map observations directly to actions, tend to overfit the training data, limiting their ability to adapt to new scenarios or longer histories. 

In robotics, we are interested in learning generalizable policies that map observations to actions. However, this objective tends to often overfit to the training data, thereby limiting the ability of learned policies to adapt to new scenarios.
% Previous policy learning methods, which map observations directly to actions, tend to overfit the training data, thereby limiting their ability to adapt to new scenarios or longer histories. 
In contrast, video generation \cite{brooks2024video,veo2024} demonstrates strong generalization to novel scenes and supports training on datasets without actions. However, effectively leveraging video data for policy learning presents challenges such as the ability to match the high temporal speed required for outputting fast, fine-grained motions.
In this section, we discuss our approach for effectively leveraging video-generation methods for robotics task. 
% significant challenges, which this work seeks to address.

% video prediction offers a more robust framework by modeling scene dynamics, including both robots and their interactions with the environment over time. .


% In contrast, video prediction offers a more robust framework by preserving scene dynamics and enabling holistic future state prediction. It generalizes better to novel scenarios and supports training on datasets without actions.

% We propose an effective video-generation method for sequential decision-making tasks in robotics.

% (\(h=4\) in our experiments)
% \(\mathbf{A}_{t} = \{a_1, \ldots, a_L\}\) (\(L=4\) in our experiments)
% and each action chunk consists of \(L\) actions, 
\smallskip \noindent \textbf{Problem Statement.}
Given a sequence of image observations \(\{\mathbf{O}_{t-h+1}, \ldots, \mathbf{O}_{t}\}\) and a sequence of action chunks \(\{\mathbf{A}_{t-h}, \ldots, \mathbf{A}_{t-1}\}\), where $h$ is the history horizon, our objective is to predict the future actions \(\{\mathbf{A}_{t}, \dots, \mathbf{A}_{t+h'-1}\}\) and observations \(\{\mathbf{O}_{t+1}, \dots, \mathbf{O}_{t+h'}\}\), where $h'$ is the future horizon. 
% Our goal is to simultaneously predict videos and actions to leverage the underlying dynamics between them, while addressing the high temporal speed demand of action modeling and high spatial resolution needed for video generation.
We note that we use a higher sampling frequency for actions compared to observations, as observations typically exhibit redundancy and minimal changes over short time intervals. Each image observation (e.g., \(\mathbf{O}_{t-3}\)) corresponds to 4 actions within an action chunk (e.g., \(\mathbf{A}_{t-4}\)) in \Cref{fig:model}.



% Previous policy learning methods primarily focus on mapping observations directly to actions. While this approach may work in controlled settings, it often leads to overfitting on the training data, making it challenging to generalize to new observations or scenarios with longer historical dependencies. In contrast, we argue that video prediction provides a more robust framework for learning dynamic interactions.

% Video prediction preserves critical scene information by capturing the temporal and spatial dynamics of the environment, which are often overlooked when focusing solely on actions. This richer representation enables better generalization to novel scenarios, as the model learns to predict future states holistically rather than relying on narrowly defined action mappings. Additionally, video prediction has the advantage of utilizing datasets that lack explicit action annotations, making it a more flexible approach for training in diverse and real-world contexts. 




% We proposed a masked video autoencoder method for performing multiple tasks including policy learning, forward dynamics prediction, inverse dynamics modeling, video-based planning, and comprehensive modeling of full dynamics.

% We explore the application of video generation models to sequential decision-making tasks in robotics. 
% Given a sequence of observations \(\{\mathbf{O}_{t-h}, \cdots, \mathbf{O}_{t}\}\) and a sequence of actions \(\{\mathbf{a}_{t-h}, \cdots, \mathbf{a}_{t}, \cdots, \mathbf{a}_{t+h}\}\), our objective is to perform several essential tasks in policy learning, dynamics modeling, and video planning.

% We propose a masked video autoencoder capable of selectively masking inputs and outputs, enabling it to perform multiple tasks. These include policy learning, forward dynamics prediction, inverse dynamics modeling, video-based planning, and comprehensive modeling of full system dynamics.

\smallskip 
\noindent\textbf{Encode History}.
We first process the historical image observations through a pre-trained VAE encoder (kl-f16) \cite{rombach2021highresolution} to obtain their latent representations. 
Each image is encoded into a latent map of dimensions \(\mathbb{R}^{w \times h \times 16}\), where \(w\) and \(h\) represent the width and height, and \(16\) is the latent dimension. For input images of size \(256 \times 256\), this results in a latent map with \(w=16\) and \(h=16\). The map is then flattened and processed by a fully-connected (FC) layer, projecting each element into a \(768\)-dimensional latent vector. Thus, the image is represented as a sequence of $N=256$ visual tokens, each with \(768\)-dimensional features.
For the action chunk with $4$ actions, it is repeated 64 times to match the number of visual tokens. The repeated sequence is then passed through an FC layer, converting it into a sequence of 256 action tokens, each with a \(768\)-dimensional latent representation.
These history visual and action tokens serve as conditions for predicting future observations and actions.

To address the problem of video action modeling, we propose a unified latent video-action representation that integrates the visual and action data. We first discuss how this latent representation can be used within a masked training objective providing flexibility for this model in~\cref{sec:mae}. We will then discuss the choice of decoupling video-action diffusion for fast inference addressing the high temporal speed demand of robot policies while balancing the high spatial resolution needed for video generation in~\cref{sec:decouple}.
% Autoencoders are neural networks that learn to compress data into a compact latent representation and reconstruct it back to its original form. They consist of an encoder, which reduces the data to a lower-dimensional space, and a decoder, which restores the data from this compressed representation. 

\subsection{Masked Autoencoder for Observation Prediction}
\label{sec:mae}
Our work is closely related to \cite{li2024autoregressive,chang2022maskgit}. Their method focuses on image generation conditioned on class labels. It begins by generating a subset of visual tokens for the image and then sequentially predicts additional tokens based on the previously generated ones, following an autoregressive process to complete the image. This step-by-step autoregressive approach has been shown to outperform single-step generation of all visual tokens simultaneously.
To facilitate step-by-step prediction, they employ a masked autoencoder framework. During training, some visual tokens are randomly masked, and the model is trained to reconstruct these masked tokens. At inference time, the model predicts the full set of tokens by iteratively generating them, starting from an empty sequence. 

We follow this setting for video prediction.
Future observation frames \(\{\mathbf{O}_{t+1}, \ldots, \mathbf{O}_{t+h}\}\) are processed similarly to historical observations: they are passed through a VAE encoder to extract latent representations, followed by an FC layer, resulting in a sequence of 256 tokens per frame, each with a \(768\)-dimensional latent vector. 
These visual tokens are concatenated channel-wise with historical visual tokens and action tokens (as shown in~\cref{fig:model}) to form a new sequence of latent features, which is then temporally concatenated with latent representations from other time steps to produce a \(256 \times 4\) latent sequence.  
The resulting sequence is passed through a Transformer to fuse information, resulting in a set of joint video-action latent representations, \(\{\mathbf{Z}_{t+1}, \ldots, \mathbf{Z}_{t+h}\}\), where each latent (e.g., \(\mathbf{Z}_{t+1}\)) contain 256 latent tokens. These latent tokens are then used to reconstruct the future observations and corresponding action chunks.


During training, we randomly mask tokens within the future observation frames and train the model to reconstruct these masked tokens. To minimize information leakage across different frames, we consistently mask the same positions across all video frames. At inference time, the model generates complete videos by predicting all tokens starting from an empty sequence. Notably, the autoregressive generation operates in the spatial domain, where visual tokens across all video frames are generated simultaneously in each step.
Unlike image generation conditioned on class labels or text, historical observations provide rich contextual information about the environment. While our model is capable of generating videos in an autoregressive manner, we have found that a single-step process is sufficient to produce high-quality future observations.


% By focusing on video prediction, models gain a deeper understanding of the dynamics, improving their adaptability and robustness across different tasks.




\subsection{Decoupled Video and Action Diffusions}
\label{sec:decouple}
Previous video-based policy learning methods rely on generating videos first and then predicting actions, leading to slow speed and accumulated errors. To address this, we propose decoupling video and action prediction while training them jointly. 
During training, video generation helps the learned latent representations capture more detailed scene information, which benefits action prediction. 
During policy inference, where speed is crucial, the decoupled design allows us to bypass video generation and decode only actions.
% This approach leverages rich scene information from videos to enhance action prediction. In addition. during inference, only actions are decoded, improving inference speed. 

We introduce two lightweight diffusion decoders for action and video prediction (see \Cref{fig:model}). Unlike prior video generation methods for policy learning, which require multiple denoising steps across the entire model, our approach confines the denoising process to the lightweight decoders, delivering more efficient performance. This design preserves the generative strengths of diffusion models while significantly reducing inference time. 

As illustrated in \Cref{fig:model}, the latent tokens \(\mathbf{Z}_{t+1}\) serve as the conditioning input for the diffusion decoders. The video diffusion decoder processes each latent token \(z_i \in \mathbf{Z}_{t+1} = \{z_1, \ldots, z_{256}\}\) to predict individual patches in the video frame, which are then reshaped and sent to the VAE decoder to reconstruct the full frame $\mathbf{O}_{t+1}$. For the action diffusion decoder, all latent tokens in \(\mathbf{Z}_{t+1}\) are aggregated using a convolutional layer, followed by an MLP layer, to produce \(L=4\) action latent. These latent are used as the conditions for a small action diffusion model to generate the action chunk $\mathbf{A}_t=\{a_1, \dots, a_L\}$. The model predicts 4 future images and 16 future actions each time, with each image corresponding to 4 actions.

During training, the decoders learn to predict the noise added to noisy action chunks or video frames. 
The action diffusion loss is defined as:
\[
\mathcal{L}_{\text{action}}(\mathbf{Z}, \mathbf{A}) = \mathbb{E}_{\epsilon, k} \left[\| \epsilon - \epsilon_\theta(\mathbf{A}_k | k, \mathbf{Z}) \|^2 \right],
\]
where \(\mathbf{A}_k\) represents the noisy actions, \(\epsilon\) is the added noise, \(k\) is the diffusion timestep, \(\mathbf{Z}\) is the joint video-action latent, and \( \epsilon_\theta(\mathbf{A}_k | k, \mathbf{Z}) \) is the predicted noise.

Similarly, the video diffusion loss is defined as:
\[
\mathcal{L}_{\text{video}}(\mathbf{Z}, \mathbf{O}) = \mathbb{E}_{\epsilon, k} \left[\frac{1}{N} \sum_{i=1}^{N} \| \epsilon_i - \epsilon_\phi(\mathbf{O}_k^i | k, \mathbf{Z}) \|^2 \right],
\]
where \( \mathbf{O}_k^i \) represents the \( i \)-th noisy visual token in the video frame \( \mathbf{O}_k \) at diffusion timestep \( k \), \( N \) is the total number of visual tokens in the video frame, \( \epsilon_i \) is the added noise to the \( i \)-th visual token, and \( \epsilon_\phi(\mathbf{O}_k^i | k, \mathbf{Z}) \) is the predicted noise for the \( i \)-th token.

% \( \epsilon_i \) is the Gaussian noise added to the \( i \)-th visual token during the forward process. \( \epsilon_\theta(\mathbf{O}_k^i | k, \mathbf{Z}) \) is the model's predicted noise for the \( i \)-th token, conditioned on \( k \) and the latent tokens \( \mathbf{Z} \).


The total loss is the combination of the action and video diffusion losses:
$\mathcal{L} = \mathcal{L}_{\text{action}} + \mathcal{L}_{\text{video}}$.
During policy inference, the decoders generate actions by iteratively refining pure noise through the learned denoising process.


\smallskip
\noindent \textbf{Masked Training with Flexbile Objectives}. 
Instead of training the model solely on the task of predicting future observations and actions based on historical data, we propose a masked training approach with multiple training objectives using a unified framework. As illustrated in \Cref{fig:overview}, the model is trained on five distinct tasks by varying input and output combinations. Unused components are masked and replaced with a learned mask token. The action loss and video loss are selectively applied to supervise the model depending on the specific task. 
This masked training strategy not only enables the model to perform a variety of tasks—serving as a robot policy, video model, forward and inverse dynamics model, and task planner—but also significantly reduces overfitting to individual tasks, enhancing its versatility and robustness.
